Trustworthy RAG: An Evaluation Agent for Detecting Misinformation and Knowledge Poisoning in Generative AI Systems

Retrieval-Augmented Generation (RAG) grounds Large Language Model (LLM) outputs in external knowledge, but RAG systems usually trust whatever they retrieve, creating a Security-Reliability Gap: high semantic relevance does not guarantee factual truth. Adversaries exploit this through knowledge poisoning, inserting malicious documents to cause targeted misinformation. We propose an Evaluation Agent, middleware that combines Natural Language Inference (NLI) factual verification, a five-signal poison detector with relevance-weighted aggregation, and a Trust Index T = 0.4 F + 0.35 C + 0.25 (1 - P ) with a non-linear dampener for high-contamination contexts. On TruthfulQA with Llama 3.3 70B, the agent reaches 91% accuracy and 100% precision, with 100% recall on instruction injection, while in-place edits, such as entity swaps, remain hard to detect. Across three LLMs the Trust Index stays discriminative, with a Receiver Operating Characteristic Area Under the Curve (ROC-AUC) of 0.73 to 0.81; generation style matters more than model size, and per-LLM threshold calibration restores baseline competitive accuracy, whereas a weaker FEVER result shows that cross-dataset generalization requires domain-specific calibration. In a software-engineering use case, a secure-coding assistant over guidance from the Open Worldwide Application Security Project (OWASP) Top 10 and the Common Weakness Enumeration (CWE), the agent reliably blocks instruction injection of unsafe advice (F1 92%), while contradiction and subtle semantic weakening remain hard. Throughout, the agent measures detection of poisoned context before generation, not whether the LLM adopts the injected misinformation. We release the proposed approach, attack generator, and experimental artifacts at the link: https://github.com/GPT-Laboratory/TrustworthyRAG.

==> roc_figure.tex <==
% Auto-generated ROC figure (requires \usepackage{pgfplots})
\begin{figure}[t]\centering\begin{tikzpicture}
\begin{axis}[width=\columnwidth,height=0.78\columnwidth,xlabel={False positive rate},ylabel={True positive rate},xmin=0,xmax=1,ymin=0,ymax=1,legend pos=south east,grid=both,font=\small]
\addplot[thick] coordinates {(0.0000,0.0000) (0.0000,0.0083) (0.0000,0.0083) (0.0000,0.0250) (0.0000,0.0250) (0.0000,0.0333) (0.0000,0.0583) (0.0000,0.0583) (0.0000,0.0583) (0.0000,0.0583) (0.0000,0.0583) (0.0000,0.0583) (0.0000,0.0917) (0.0000,0.1000) (0.0000,0.1250) (0.0000,0.1250) (0.0000,0.2083) (0.0000,0.2500) (0.0000,0.3083) (0.0000,0.3500) (0.0000,0.3750) (0.0015,0.3750) (0.0029,0.3833) (0.0029,0.4083) (0.0029,0.4083) (0.0029,0.4167) (0.0059,0.4167) (0.0088,0.4500) (0.0088,0.4750) (0.0088,0.4917) (0.0088,0.5167) (0.0191,0.5167) (0.0191,0.5167) (0.0206,0.5583) (0.0206,0.5583) (0.0294,0.5667) (0.0426,0.5750) (0.0500,0.5750) (0.0618,0.5750) (0.0691,0.5750) (0.1191,0.5750) (0.1412,0.6000) (0.1735,0.6417) (0.2309,0.6833) (0.2971,0.6833) (0.3691,0.7333) (0.4632,0.7833) (0.5235,0.8167) (0.5706,0.8500) (0.6382,0.8917) (0.6912,0.9667) (0.7471,0.9917) (0.8147,0.9917) (0.8338,1.0000) (0.8824,1.0000) (0.9294,1.0000) (0.9559,1.0000) (0.9632,1.0000) (0.9706,1.0000) (0.9779,1.0000) (1.0000,1.0000) (1.0000,1.0000)};
\addlegendentry{Llama 3.3 70B (AUC=0.81)}
\addplot[thick,dashed] coordinates {(0.0000,0.0000) (0.0000,0.0333) (0.0000,0.0333) (0.0000,0.0667) (0.0000,0.1000) (0.0000,0.1333) (0.0000,0.2000) (0.0000,0.2000) (0.0000,0.2000) (0.0000,0.2333) (0.0000,0.2667) (0.0000,0.2667) (0.0000,0.2667) (0.0000,0.2667) (0.0000,0.3000) (0.0000,0.3000) (0.0000,0.3000) (0.0000,0.3000) (0.0294,0.3000) (0.0608,0.4000) (0.0980,0.4000) (0.1549,0.4333) (0.2118,0.4333) (0.2176,0.5000) (0.2412,0.5333) (0.2647,0.5333) (0.2882,0.6000) (0.3176,0.6667) (0.3451,0.7333) (0.4216,0.7333) (0.4627,0.7667) (0.5235,0.7667) (0.5529,0.7667) (0.5922,0.8333) (0.6157,0.8333) (0.6275,0.8333) (0.6294,0.8333) (0.6431,0.8333) (0.6569,0.8667) (0.6706,0.8667) (0.6706,0.8667) (0.6784,0.8667) (0.6784,0.8667) (0.6902,0.9000) (0.7118,0.9000) (0.7451,0.9000) (0.7765,0.9333) (0.8098,0.9333) (0.8353,0.9333) (0.8529,0.9333) (0.8765,0.9333) (0.8804,0.9667) (0.8922,0.9667) (0.9020,0.9667) (0.9118,1.0000) (0.9353,1.0000) (0.9392,1.0000) (0.9451,1.0000) (0.9725,1.0000) (0.9961,1.0000) (1.0000,1.0000) (1.0000,1.0000)};
\addlegendentry{Qwen 3.5 35B (AUC=0.73)}
\addplot[thick,dash dot] coordinates {(0.0000,0.0000) (0.0000,0.0667) (0.0000,0.0667) (0.0000,0.1333) (0.0000,0.2000) (0.0000,0.2000) (0.0000,0.2000) (0.0000,0.3333) (0.0000,0.3333) (0.0118,0.3333) (0.0118,0.4000) (0.0118,0.4000) (0.0235,0.4000) (0.0235,0.4000) (0.0235,0.4000) (0.0235,0.4000) (0.0471,0.4000) (0.0471,0.4000) (0.0706,0.4000) (0.0706,0.4000) (0.0824,0.4667) (0.0941,0.4667) (0.1059,0.4667) (0.1294,0.5333) (0.1529,0.5333) (0.1647,0.5333) (0.1765,0.5333) (0.1765,0.5333) (0.1765,0.6000) (0.1882,0.6000) (0.2000,0.6000) (0.2118,0.6000) (0.2235,0.6000) (0.2353,0.6000) (0.2353,0.6667) (0.2471,0.6667) (0.2588,0.7333) (0.2941,0.8000) (0.3059,0.8000) (0.3059,0.8000) (0.3529,0.8000) (0.4000,0.8000) (0.4353,0.8000) (0.4941,0.8000) (0.5765,0.8000) (0.6000,0.8000) (0.6235,0.8667) (0.6706,0.8667) (0.6824,0.9333) (0.7059,1.0000) (0.7294,1.0000) (0.7765,1.0000) (0.8000,1.0000) (0.8118,1.0000) (0.8588,1.0000) (0.9412,1.0000) (0.9647,1.0000) (0.9647,1.0000) (0.9882,1.0000) (0.9882,1.0000) (1.0000,1.0000) (1.0000,1.0000)};
\addlegendentry{Mistral 7B Instruct (AUC=0.79)}
\addplot[gray,dotted] coordinates {(0,0)(1,1)};
\end{axis}\end{tikzpicture}
\caption{ROC curves for poison detection on pooled mixed-strategy runs. Per-LLM calibration improves the usable operating point (Table~\ref{tab:calib}).}\label{fig:roc}\end{figure}

==> strategy_bar_figure.tex <==
% Auto-generated: per-strategy detection bar chart (requires pgfplots)
\begin{figure}[t]\centering\begin{tikzpicture}
\begin{axis}[width=\columnwidth,height=0.62\columnwidth,ybar,bar width=6pt,
    ymin=0,ymax=105,ylabel={Score (\%)},symbolic x coords={Injection,Contradict.,Subtle,Entity swap,Mixed},
    xtick=data,x tick label style={font=\footnotesize,rotate=20,anchor=east},
    legend pos=north east,legend style={font=\footnotesize},ymajorgrids,font=\small]
\addplot[fill=blue!55] coordinates {(Injection,100.0) (Contradict.,53.3) (Subtle,20.0) (Entity swap,3.3) (Mixed,40.0)};
\addplot[fill=orange!70] coordinates {(Injection,96.8) (Contradict.,68.1) (Subtle,33.3) (Entity swap,5.9) (Mixed,56.1)};
\legend{Recall, F1}
\end{axis}\end{tikzpicture}
\caption{Per-strategy detection on TruthfulQA (Llama~3.3~70B + MiniLM, $K{=}5$): the hierarchy injection $\gg$ contradiction $\gg$ subtle $\approx$ entity swap.}\label{fig:strategybar}\end{figure}

==> trust_dist_figure.tex <==
% Auto-generated: clean vs poisoned trust-score distribution (pgfplots)
\begin{figure}[t]\centering\begin{tikzpicture}
\begin{axis}[width=\columnwidth,height=0.62\columnwidth,ybar,bar width=4pt,
    xmin=0,xmax=1,ymin=0,ymax=0.45,xlabel={Trust Index $T$},ylabel={Fraction of samples},
    legend pos=north west,legend style={font=\footnotesize},ymajorgrids,font=\small]
\addplot[fill=green!45] coordinates {(0.05,0.000) (0.15,0.000) (0.25,0.000) (0.35,0.000) (0.45,0.005) (0.55,0.024) (0.65,0.042) (0.75,0.306) (0.85,0.400) (0.95,0.224)};
\addplot[fill=red!55] coordinates {(0.05,0.000) (0.15,0.027) (0.25,0.027) (0.35,0.213) (0.45,0.133) (0.55,0.093) (0.65,0.067) (0.75,0.187) (0.85,0.253) (0.95,0.000)};
\draw[dashed,thick] (axis cs:0.5,0) -- (axis cs:0.5,0.45);
\legend{Clean, Poisoned}
\end{axis}\end{tikzpicture}
\caption{Trust Index distribution for clean vs poisoned (TruthfulQA mixed, Llama~3.3~70B + MiniLM, $K{=}5$); dashed line marks the threshold $\tau{=}0.5$.}
\label{fig:trustdist}
\end{figure}
